CogCompTime: A Tool for Understanding Time in Natural Language Text

Automatic extraction of temporal information in text is an important component of natural language understanding. It involves two basic tasks: (1) Understanding time expressions that are mentioned explicitly in text (e.g., February 27, 1998 or tomorrow), and (2) Understanding temporal information that is conveyed implicitly via relations. In this paper, we introduce CogCompTime, a system that has these two important functionalities. It incorporates the most recent progress, achieves state-of-the-art performance, and is publicly available.1 We believe that this demo will be useful for multiple time-aware applications and provide valuable insight for future research in temporal understanding.

==> related.tex <==
% !TEX root = root.tex
\ignore{
\section{Background}
\label{sec:related}
In practice, TempRels are usually more common than Timexes:
According to the dataset provided by the TempEval3 workshop \cite{ULADVP13}, there are 2 Timexes and 12 TempRels in every 100 tokens on average.
}
